A coefficient related to splay-to-root traversal, correct to thousands of decimal places

This paper takes another look at the cost of traversing a binary tree using repeated splay-to-root. This was shown to cost $O(n)$ (in rotations) by Tarjan and later, in different ways, by Elmasry and others. It would be interesting to know the minimal possible coefficient implied by the $O(n)$ cost; call this coefficient $\beta$. In this paper we define a related coefficient $\alpha$ describing the cost of splay-to-root traversal on maximal (i.e., complete) binary trees, and show that $\beta \geq 2 + \alpha$. We give the first 3009 digits of $\alpha$, including the decimal point, and show that every digit is correct. We make two conjectures: first, that $\beta = 2 + \alpha$, and second, that $\alpha$ is irrational.

==> figures/oldfigechelon <==
#FIG 3.2  Produced by xfig version 3.2.5c
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
6 11100 2895 11565 3390
4 0 0 50 -1 1 30 0.0000 4 330 300 11100 3225 A\001
4 0 0 50 -1 0 20 0.0000 4 225 165 11400 3390 0\001
-6
6 11835 1605 12240 1965
4 0 0 50 -1 1 30 0.0000 4 210 225 11835 1815 x\001
4 0 0 50 -1 0 20 0.0000 4 225 165 12075 1965 0\001
-6
6 10260 1320 10680 1695
4 0 0 50 -1 1 30 0.0000 4 210 225 10260 1530 x\001
4 0 0 50 -1 0 20 0.0000 4 225 165 10515 1695 1\001
-6
6 9330 2115 9780 2550
4 0 0 50 -1 1 30 0.0000 4 210 225 9330 2325 x\001
4 0 0 50 -1 0 20 0.0000 4 225 165 9615 2550 2\001
-6
6 10275 3030 10695 3480
4 0 0 50 -1 1 30 0.0000 4 330 300 10275 3360 A\001
4 0 0 50 -1 0 20 0.0000 4 225 165 10530 3480 1\001
-6
6 9165 3015 9600 3465
4 0 0 50 -1 1 30 0.0000 4 330 300 9165 3345 A\001
4 0 0 50 -1 0 20 0.0000 4 225 165 9435 3465 2\001
-6
6 8295 3060 8730 3510
4 0 0 50 -1 1 30 0.0000 4 330 300 8295 3390 A\001
4 0 0 50 -1 0 20 0.0000 4 225 165 8565 3510 3\001
-6
6 7605 2955 8040 3450
4 0 0 50 -1 1 30 0.0000 4 330 300 7605 3285 A\001
4 0 0 50 -1 0 20 0.0000 4 225 165 7875 3450 4\001
-6
6 7020 2910 7455 3405
4 0 0 50 -1 1 30 0.0000 4 330 300 7020 3240 A\001
4 0 0 50 -1 0 20 0.0000 4 240 165 7290 3405 5\001
-6
6 6330 2775 6735 3270
4 0 0 50 -1 1 30 0.0000 4 330 300 6330 3105 A\001
4 0 0 50 -1 0 20 0.0000 4 225 165 6570 3270 6\001
-6
6 2805 2295 3270 2790
4 0 0 50 -1 1 30 0.0000 4 330 300 2805 2625 A\001
4 0 0 50 -1 0 20 0.0000 4 225 165 3105 2790 0\001
-6
6 2385 2985 2805 3435
4 0 0 50 -1 1 30 0.0000 4 330 300 2385 3315 A\001
4 0 0 50 -1 0 20 0.0000 4 225 165 2640 3435 1\001
-6
6 1935 3600 2370 4050
4 0 0 50 -1 1 30 0.0000 4 330 300 1935 3930 A\001
4 0 0 50 -1 0 20 0.0000 4 225 165 2205 4050 2\001
-6
6 3000 1230 3405 1590
4 0 0 50 -1 1 30 0.0000 4 210 225 3000 1440 x\001
4 0 0 50 -1 0 20 0.0000 4 225 165 3240 1590 0\001
-6
6 1740 1665 2160 2040
4 0 0 50 -1 1 30 0.0000 4 210 225 1740 1875 x\001
4 0 0 50 -1 0 20 0.0000 4 225 165 1995 2040 1\001
-6
6 1350 2205 1800 2640
4 0 0 50 -1 1 30 0.0000 4 210 225 1350 2415 x\001
4 0 0 50 -1 0 20 0.0000 4 225 165 1635 2640 2\001
-6
6 990 2835 1395 3240
4 0 0 50 -1 1 30 0.0000 4 210 225 990 3045 x\001
4 0 0 50 -1 0 20 0.0000 4 225 165 1230 3240 3\001
-6
6 7965 825 8370 1230
4 0 0 50 -1 1 30 0.0000 4 210 225 7965 1035 x\001
4 0 0 50 -1 0 20 0.0000 4 225 165 8205 1230 3\001
-6
6 8160 2355 8640 2700
4 0 0 50 -1 1 30 0.0000 4 210 225 8160 2565 x\001
4 0 0 50 -1 0 20 0.0000 4 225 165 8475 2700 4\001
-6
6 7185 1815 7530 2250
4 0 0 50 -1 1 30 0.0000 4 210 225 7185 2025 x\001
4 0 0 50 -1 0 20 0.0000 4 240 165 7365 2250 5\001
-6
6 6645 2145 7050 2580
4 0 0 50 -1 1 30 0.0000 4 210 225 6645 2355 x\001
4 0 0 50 -1 0 20 0.0000 4 225 165 6885 2580 6\001
-6
6 5985 870 6360 1245
6 5985 870 6360 1245
4 0 0 50 -1 1 30 0.0000 4 210 225 5985 1080 x\001
4 0 0 50 -1 0 20 0.0000 4 225 165 6195 1245 7\001
-6
-6
1 3 0 1 0 7 50 -1 0 0.000 1 0.0000 11640 2085 75 75 11640 2085 11640 2160
1 3 0 1 0 7 50 -1 0 0.000 1 0.0000 10005 2505 75 75 10005 2505 10005 2580
1 3 0 1 0 7 50 -1 0 0.000 1 0.0000 10305 1815 75 75 10305 1815 10305 1890
1 3 0 1 0 7 50 -1 0 0.000 1 0.0000 7950 1365 75 75 7950 1365 7950 1440
1 3 0 1 0 7 50 -1 0 0.000 1 0.0000 7635 2310 75 75 7635 2310 7635 2385
1 3 0 1 0 7 50 -1 0 0.000 1 0.0000 7935 2580 75 75 7935 2580 7935 2655
1 3 0 1 0 7 50 -1 0 0.000 1 0.0000 7245 2490 75 75 7245 2490 7245 2565
1 3 0 1 0 7 50 -1 0 0.000 1 0.0000 6630 1125 75 75 6630 1125 6630 1200
1 3 0 1 0 7 50 -1 0 0.000 1 0.0000 7245 300 75 75 7245 300 7245 375
1 3 0 1 0 7 50 -1 0 0.000 1 0.0000 3195 825 75 75 3195 825 3195 900
1 3 0 1 0 7 50 -1 0 0.000 1 0.0000 2805 1350 75 75 2805 1350 2805 1425
1 3 0 1 0 7 50 -1 0 0.000 1 0.0000 2370 1980 75 75 2370 1980 2370 2055
1 3 0 1 0 7 50 -1 0 0.000 1 0.0000 1965 2550 75 75 1965 2550 1965 2625
1 3 0 1 0 7 50 -1 0 0.000 1 0.0000 1545 3165 75 75 1545 3165 1545 3240
2 1 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 3
	 6630 1110 11655 2070 11340 2685
2 1 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 3
	 10335 1815 10005 2490 9510 2955
2 1 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9990 2505 10170 2985
2 1 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 3
	 7980 1350 7650 2280 6660 2775
2 1 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7650 2280 8415 2985
2 1 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7260 2490 7350 2835
2 1 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7935 2565 7695 2880
2 1 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 5775 2220 7275 300
2 1 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 3195 810 1140 3735
2 1 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 2385 1965 2715 2445
2 1 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 1978 2546 2308 3026
2 1 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 1543 3131 1873 3611
4 0 0 50 -1 1 30 0.0000 4 315 225 3330 900 y\001
4 0 0 50 -1 1 30 0.0000 4 315 225 7320 360 y\001

